UniLumos: Fast and Unified Image and Video Relighting with Physics-Plausible Feedback

Relighting is a crucial task with both practical demand and artistic value, and recent diffusion models have shown strong potential by enabling rich and controllable lighting effects. However, as they are typically optimized in semantic latent space, where proximity does not guarantee physical correctness in visual space, they often produce unrealistic results, such as overexposed highlights, misaligned shadows, and incorrect occlusions. We address this with UniLumos, a unified relighting framework for both images and videos that brings RGB-space geometry feedback into a flow matching backbone. By supervising the model with depth and normal maps extracted from its outputs, we explicitly align lighting effects with the scene structure, enhancing physical plausibility. Nevertheless, this feedback requires high-quality outputs for supervision in visual space, making standard multi-step denoising computationally expensive. To mitigate this, we employ path consistency learning, allowing supervision to remain effective even under few-step training regimes. To enable fine-grained relighting control and supervision, we design a structured six-dimensional annotation protocol capturing core illumination attributes. Building upon this, we propose LumosBench, a disentangled attribute-level benchmark that evaluates lighting controllability via large vision-language models, enabling automatic and interpretable assessment of relighting precision across individual dimensions. Extensive experiments demonstrate that UniLumos achieves state-of-the-art relighting quality with significantly improved physical consistency, while delivering a 20x speedup for both image and video relighting. Code is available at https://github.com/alibaba-damo-academy/Lumos-Custom.

==> damo_camera_ready_arxiv/tab_1.tex <==
\begin{table*}[t]
\centering
\caption{Quantitative comparison. \textbf{Bold} number indicate the best performance.}
\label{main_results}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|c|cc}
\toprule
\multirow{2}{*}{\textbf{Model}} & 
\multicolumn{3}{c|}{\textbf{(a) Quality}} & \textbf{(b) Temporal Consistency} & \multicolumn{2}{c}{\textbf{(c) Lumos Consistency}}\\
& PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ 
& R-Motion$\downarrow$ & Avg. Score $\uparrow$ & Dense L2 Error $\downarrow$ \\
\midrule
\multicolumn{7}{c}{\textbf{Image Relighting}}\\
\midrule
SwitchLight \cite{kim2024switchlight}      
&20.483 &0.901 &0.094&-  &0.717&0.388\\
DiLightNet  \cite{zeng2024dilightnet}      
&21.894 &0.860 &0.131 &-  &0.682&0.401\\
IC-Light    \cite{zhang2025scaling}        
&24.316 &0.884 &0.108 &-  &0.703&0.447\\
SynthLight \cite{chaturvedi2025synthlight} 
&25.572 &0.905 &0.102 &-  &0.791&0.214\\
\midrule
\rowcolor{blue!10}  
\textbf{UniLumos} 
&\textbf{26.719} & \textbf{0.913} & \textbf{0.089} &- &\textbf{0.912} &\textbf{0.103}\\
\midrule
\multicolumn{7}{c}{\textbf{Video Relighting}}\\
\midrule
IC-Light Per Frame  \cite{zhang2025scaling} 
&20.132 &0.851 &0.133 &2.437 &0.672&0.432\\
Light-A-Video \cite{zhou2025light} + CogVideoX\cite{yang2024cogvideox}
&19.851 &0.859 &0.124 &1.784 &0.641&0.383\\
Light-A-Video \cite{zhou2025light}  + Wan2.1\cite{wan2025}
&20.784 &0.876 &0.129 &1.582 &0.682&0.371\\
\midrule
\rowcolor{blue!10}  
\textbf{UniLumos}                   
&\textbf{25.031} &\textbf{0.891} &\textbf{0.109} &\textbf{1.436} &\textbf{0.871} &\textbf{0.147}\\
\bottomrule
\end{tabular}
}
\end{table*}

==> damo_camera_ready_arxiv/tab_2.tex <==
\begin{table*}[t]
\centering
% \vspace{-2mm}
\caption{Quantitative comparison. \textbf{Bold} number indicate the best performance.}
\label{main_results_ab}
%\vspace{-2mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|c|cc}
\toprule
\multirow{2}{*}{\textbf{Model}} & 
\multicolumn{3}{c|}{\textbf{(a) Quality}} & \textbf{(b) Temporal Consistency} & \multicolumn{2}{c}{\textbf{(c) Lumos Consistency}}\\
& PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ 
& R-Motion$\downarrow$ & Avg. Score $\uparrow$ & Dense L2 Error $\downarrow$ \\
\midrule
\multicolumn{7}{c}{\textbf{Ablative Study}}\\
\midrule
w/o Depth Feedback   &23.472 &0.883 &0.118   &1.443 &0.870 &0.265\\
w/o Normal Feedback  &22.115 &0.874 &0.123   &1.446 &0.863 &0.173\\
w/o All Feedback     &21.433 &0.862 &0.139   &1.473 &0.859 &0.297\\
w/o Path Consistency &\textbf{25.317} &\textbf{0.902} &0.113 &1.438 &\textbf{0.875}&0.153\\
\midrule
\multicolumn{7}{c}{\textbf{Effect of Training Domain}}\\
\midrule
Only Video          &22.487&0.863&0.119&1.487&0.857&0.173\\
Only Image          &24.471&0.872&0.123&2.429&0.841&0.182\\
\midrule
\rowcolor{blue!10}  
\textbf{UniLumos} &25.031 &0.891 &\textbf{0.109} &\textbf{1.436}&0.871&\textbf{0.147}\\
\bottomrule
\end{tabular}
}
% \vspace{-4mm}
\end{table*}

==> damo_camera_ready_arxiv/tab_3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\centering
\vspace{-2mm}
\caption{Quantitative comparison of the attribute-level controllability. \textbf{Bold} number indicate the best performance.}
%\vspace{-2mm}
\label{main_results_lumos_ab}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cccccc|c}
\toprule
\textbf{Model} 
&\#Params 
&Direction   
&Light Source Type 
& Intensity & Color Temperature & Temporal Dynamics & Optical Phenomena & Avg. Score \\ 
\midrule
\multicolumn{9}{c}{\textbf{General Models}}\\
\midrule
LTX-Video \cite{hacohen2024ltx}          &1.9B &0.794&0.644&0.487&0.708&0.487&0.403&0.587\\
CogVideoX \cite{yang2024cogvideox}       &5.6B &0.837&0.692&0.552&0.739&0.532&0.449&0.634\\
HunyuanVideo \cite{kong2024hunyuanvideo} &13B  &0.863&0.741&0.599&0.802&0.655&0.481&0.690\\
Wan2.1\cite{wan2025}                    &1.3B  &0.842&0.685&0.436&0.741&0.504&0.433&0.607\\
Wan2.1\cite{wan2025}                    &14B &0.871&0.794&0.674&\textbf{0.829}&\textbf{0.737}&0.505&0.735\\
\midrule
\multicolumn{9}{c}{\textbf{Specialized Models}}\\
\midrule
IC-Light Per-Frame  
\cite{zhang2025scaling} 
&0.9B &0.793&0.547&0.349&0.493&0.284&0.339&0.468\\
Light-A-Video \cite{zhou2025light} + CogVideoX\cite{yang2024cogvideox}
&2.9B &0.787&0.581&0.327&0.536&0.493 &0.373 &0.516\\
Light-A-Video \cite{zhou2025light} + Wan2.1\cite{wan2025}
&2.2B&0.801&0.603&0.361&0.582&0.557 &0.412 &0.553\\
\midrule
\textbf{UniLumos} w/o lumos captions 
&1.3B &0.868&0.774&0.529&0.798&0.543&0.457&0.662\\
\rowcolor{blue!10}
\textbf{UniLumos} 
&1.3B &\textbf{0.893}&\textbf{0.847}&\textbf{0.832}&0.813&0.662&\textbf{0.592}&\textbf{0.773}\\
\bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{table*}

==> damo_camera_ready_arxiv/tab_notions.tex <==
% \begin{table*}[t]
% \centering
% \caption{Classification criteria and definitions for light-related scene attributes.}
% \label{tab:light-attributes}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|c|c}
% \toprule
% \textbf{Primary Category} & \textbf{Subcategory} & \textbf{Definition} \\
% \midrule
% \multirow{7}{*}{Direction of Light} 
%   & Front Light & The light source is positioned directly in front of the subject, illuminating it head-on. \\
  
%   & Side Light & The light source is positioned at a 90-degree or 45-degree angle to the subject, coming from the side. \\
  
%   & Back Light & The light source is located behind the subject, directed towards the camera. \\
  
%   & Top Light & The light source is positioned directly above the subject, casting light downwards. \\
  
%   & Bottom Light & The light source is positioned below the subject, casting light upwards. \\
  
%   & Split Light & The light source illuminates one side of the subject while leaving the other side in shadow. \\
  
%   & Ambient Light Without Clear Direction & Ambient light is non-directional, uniformly illuminating the environment from multiple sources. \\
% \midrule
% \multirow{3}{*}{Light Source Type}
%   & Natural Light & Illumination from nature without human intervention, varying with time of day, weather, and location. \\
  
%   & Artificial Light & Human-made light sources (e.g., bulbs, LEDs) used in indoor/outdoor spaces for functional or artistic effects. \\
  
%   & Rendering Light & Digitally simulated light in CGI, games, or animations using techniques like ray tracing. \\
% \midrule
% \multirow{3}{*}{Light Intensity}
%   & Glare & Extremely bright light over 1000 lumens that can cause discomfort or obscure detail. \\
%   & Moderate & Balanced lighting (200–1000 lumens), suitable for most activities and comfortable viewing. \\
  
%   & Dim & Low lighting under 200 lumens, often cozy but may reduce visibility and detail recognition. \\
% \midrule
% \multirow{3}{*}{Color Temperature}
%   & Cool Tone & 5000K–10000K; bluish hues, common in daylight or overcast scenes. \\
  
%   & Neutral & 4000K–5000K; balanced light with no strong blue or yellow tint. \\
  
%   & Warm Tone & 2000K–4000K; reddish or yellowish hues, typical in sunrise/sunset or indoor lighting. \\
% \midrule
% \multirow{3}{*}{Light Changes in Time}
%   & Static Light & Illumination remains constant in both intensity and direction over time. \\
  
%   & Dynamic Light (Intensity Changing) & Light intensity changes gradually over time (e.g., dawn to daylight). \\
  
%   & Dynamic Light (Moving Source) & Direction of light changes due to movement of light source (e.g., headlights, stage lights). \\
% \midrule
% \multirow{4}{*}{Optical Phenomena}
%   & Transmission (Glass) & Light passes through transparent materials like glass, with possible scattering or absorption. \\
  
%   & Refraction/Reflection (Water Surface, Mirror) & Light bends or reflects at water or mirror surfaces, altering its direction. \\
  
%   & Scattering (Fog Effect) & Light diffuses through particles like fog or mist, reducing visibility. \\
  
%   & None & No significant optical phenomena are observed in the scene. \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{Classification criteria and definitions for light-related scene attributes.}
% \label{tab:light-attributes}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{>{\columncolor{paleblue}}c|>{\columncolor{palegreen}}c|>{\columncolor{palecream}}c}
% \toprule
% \textbf{Primary Category} & \textbf{Subcategory} & \textbf{Definition} \\
% \midrule
% \multirow{7}{*}{Direction of Light} 
%   & Front Light & The light source is positioned directly in front of the subject, illuminating it head-on. \\
  
%   & Side Light & The light source is positioned at a 90-degree or 45-degree angle to the subject, coming from the side. \\
  
%   & Back Light & The light source is located behind the subject, directed towards the camera. \\
  
%   & Top Light & The light source is positioned directly above the subject, casting light downwards. \\
  
%   & Bottom Light & The light source is positioned below the subject, casting light upwards. \\
  
%   & Split Light & The light source illuminates one side of the subject while leaving the other side in shadow. \\
  
%   & Ambient Light Without Clear Direction & Ambient light is non-directional, uniformly illuminating the environment from multiple sources. \\
% \midrule
% \multirow{3}{*}{Light Source Type}
%   & Natural Light & Illumination from nature without human intervention, varying with time of day, weather, and location. \\
  
%   & Artificial Light & Human-made light sources (e.g., bulbs, LEDs) used in indoor/outdoor spaces for functional or artistic effects. \\
  
%   & Rendering Light & Digitally simulated light in CGI, games, or animations using techniques like ray tracing. \\
% \midrule
% \multirow{3}{*}{Light Intensity}
%   & Glare & Extremely bright light over 1000 lumens that can cause discomfort or obscure detail. \\
%   & Moderate & Balanced lighting (200–1000 lumens), suitable for most activities and comfortable viewing. \\
  
%   & Dim & Low lighting under 200 lumens, often cozy but may reduce visibility and detail recognition. \\
% \midrule
% \multirow{3}{*}{Color Temperature}
%   & Cool Tone & 5000K–10000K; bluish hues, common in daylight or overcast scenes. \\
  
%   & Neutral & 4000K–5000K; balanced light with no strong blue or yellow tint. \\
  
%   & Warm Tone & 2000K–4000K; reddish or yellowish hues, typical in sunrise/sunset or indoor lighting. \\
% \midrule
% \multirow{3}{*}{Light Changes in Time}
%   & Static Light & Illumination remains constant in both intensity and direction over time. \\
  
%   & Dynamic Light (Intensity Changing) & Light intensity changes gradually over time (e.g., dawn to daylight). \\
  
%   & Dynamic Light (Moving Source) & Direction of light changes due to movement of light source (e.g., headlights, stage lights). \\
% \midrule
% \multirow{4}{*}{Optical Phenomena}
%   & Transmission (Glass) & Light passes through transparent materials like glass, with possible scattering or absorption. \\
  
%   & Refraction/Reflection (Water Surface, Mirror) & Light bends or reflects at water or mirror surfaces, altering its direction. \\
  
%   & Scattering (Fog Effect) & Light diffuses through particles like fog or mist, reducing visibility. \\
  
%   & None & No significant optical phenomena are observed in the scene. \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

\begin{table*}[h]
\centering
\caption{Classification criteria and definitions for light-related scene attributes.}
\label{tab:light-attributes}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|>{\columncolor{palegreen}}c|>{\columncolor{palecream}}c}
\toprule
\textbf{Primary Category} & \textbf{Subcategory} & \textbf{Definition} \\
\midrule
\multirow{7}{*}{Direction of Light} 
  & Front Light & The light source is positioned directly in front of the subject, illuminating it head-on. \\  
  & Side Light & The light source is positioned at a 90-degree or 45-degree angle to the subject, coming from the side. \\
  & Back Light & The light source is located behind the subject, directed towards the camera. \\
  & Top Light & The light source is positioned directly above the subject, casting light downwards. \\
  & Bottom Light & The light source is positioned below the subject, casting light upwards. \\
  & Split Light & The light source illuminates one side of the subject while leaving the other side in shadow. \\
  & Ambient Light Without Clear Direction & Ambient light is non-directional, uniformly illuminating the environment from multiple sources. \\
\midrule
\multirow{3}{*}{Light Source Type}
  & Natural Light & Illumination from nature without human intervention, varying with time of day, weather, and location. \\
  & Artificial Light & Human-made light sources (e.g., bulbs, LEDs) used in indoor/outdoor spaces for functional or artistic effects. \\
  & Rendering Light & Digitally simulated light in CGI, games, or animations using techniques like ray tracing. \\
\midrule
\multirow{3}{*}{Light Intensity}
  & Glare & Extremely bright light over 1000 lumens that can cause discomfort or obscure detail. \\
  & Moderate & Balanced lighting (200–1000 lumens), suitable for most activities and comfortable viewing. \\
  & Dim & Low lighting under 200 lumens, often cozy but may reduce visibility and detail recognition. \\
\midrule
\multirow{3}{*}{Color Temperature}
  & Cool Tone & 5000K–10000K; bluish hues, common in daylight or overcast scenes. \\
  & Neutral & 4000K–5000K; balanced light with no strong blue or yellow tint. \\
  & Warm Tone & 2000K–4000K; reddish or yellowish hues, typical in sunrise/sunset or indoor lighting. \\
\midrule
\multirow{3}{*}{Light Changes in Time}
  & Static Light & Illumination remains constant in both intensity and direction over time. \\
  & Dynamic Light (Intensity Changing) & Light intensity changes gradually over time (e.g., dawn to daylight). \\
  & Dynamic Light (Moving Source) & Direction of light changes due to movement of light source (e.g., headlights, stage lights). \\
\midrule
\multirow{4}{*}{Optical Phenomena}
  & Transmission (Glass) & Light passes through transparent materials like glass, with possible scattering or absorption. \\
  & Refraction/Reflection (Water Surface, Mirror) & Light bends or reflects at water or mirror surfaces, altering its direction. \\
  & Scattering (Fog Effect) & Light diffuses through particles like fog or mist, reducing visibility. \\
  & None & No significant optical phenomena are observed in the scene. \\
\bottomrule
\end{tabular}
}
\end{table*}
